Shockwave: Fair and Efficient Cluster Scheduling for Dynamic Adaptation in Machine Learning

Dynamic adaptation has become an essential technique in accelerating distributed machine learning (ML) training. Recent studies have shown that dynamically adjusting model structure (e.g., lottery ticket hypothesis) or hyperparameters (e.g., batch size) can significantly accelerate training without sacrificing accuracy. However, existing ML cluster schedulers are not designed to handle dynamic adaptation. We show that existing schemes fail to provide fairness and degrade system efficiency when the training throughput changes over time under dynamic adaptation. We design Shockwave, a scheduler with future planning that builds on two key ideas. First, Shockwave extends classic market theory from static settings to dynamic settings to co-optimize efficiency and fairness. Second, Shockwave utilizes stochastic dynamic programming to handle dynamic changes. We build a system for Shockwave and validate its performance with both trace-driven simulation and cluster experiments. Results show that for traces of ML jobs with dynamic adaptation, Shockwave improves makespan by 1.3X and fairness by 2X when compared with existing fair scheduling schemes.

==> apdx_adaptive_filter.tex <==
\section{Themis Example - Adaptive vs. Static Filter}\label{apdx:adaptive_filter}

Figure~\ref{fig:adaptive_vs_static_filter_1} and Figure~\ref{fig:adaptive_vs_static_filter_2} detail the cluster and job setting, and schedules for Table~\ref{tab:example_filter_1} and Table~\ref{tab:example_filter_2}, respectively.

\begin{figure*}[htbp!]
\centering
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[trim=0.05cm 0.1cm 0.1cm 0.1cm, clip, width=\textwidth]{figures/af1-1.png}
    \caption{Adaptive filter $f$=$1/3$ or $2/3$ or $1$.}\label{fig:af1-1}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[trim=0.05cm 0.1cm 0.1cm 0.1cm, clip, width=\textwidth]{figures/af1-2.png}
    \caption{Static filter $f$=$1/3$, one job is filtered.}\label{fig:af1-2}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[trim=0.05cm 0.1cm 0.1cm 0.1cm, clip, width=\textwidth]{figures/af1-3.png}
    \caption{Static filter $f$=$2/3$, two jobs are filtered.}\label{fig:af1-3}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[trim=0.05cm 0.1cm 0.1cm 0.1cm, clip, width=\textwidth]{figures/af1-4.png}
    \caption{Static filter $f$=1, all three jobs are filtered.}\label{fig:af1-4}
\end{subfigure}
\caption{Themis Example A (Table~\ref{tab:example_filter_1}). Comparing adaptive filter with static filter. In each round, jobs filtered or selected for allocation are shaded. Non-shaded jobs in each round are work-conserving jobs that receive left-over GPUs that are not-allocated to the filtered jobs (see leftover allocation in Themis\cite{themis20}). Cluster setting: 4 GPUs. Jobs: A, B, C are three DNN training jobs with one iteration. Serial iteration time for A, B and C are 12, 8 and 6, respectively. The number of requested GPUs per iteration for A, B and C are 3, 2 and 2, respectively. In (a) - (d), the resulting FTF-$rho$ for the three jobs are (0.78, 0.83, 0.67), (0.78, 1.0, 0.89), (0.78, 0.83, 1.1), and (0.78, 1.0, 1.1), respectively. As assumed in Themis \cite{themis20}, we adopt a linear slowdown per iteration when the number of allocated GPUs are less than the request.}\label{fig:adaptive_vs_static_filter_1}
\end{figure*}


\begin{figure*}[htbp!]
\centering
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[trim=0.05cm 0.1cm 0.1cm 0.1cm, clip, width=\textwidth]{figures/af2-1.png}
    \caption{Adaptive filter $f$=$1/3$ or $2/3$ or $1$.}\label{fig:af2-1}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[trim=0.05cm 0.1cm 0.1cm 0.1cm, clip, width=\textwidth]{figures/af2-2.png}
    \caption{Static filter $f$=$1/3$, one job is filtered.}\label{fig:af2-2}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[trim=0.05cm 0.1cm 0.1cm 0.1cm, clip, width=\textwidth]{figures/af2-3.png}
    \caption{Static filter $f$=$2/3$, two jobs are filtered.}\label{fig:af2-3}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[trim=0.05cm 0.1cm 0.1cm 0.1cm, clip, width=\textwidth]{figures/af2-4.png}
    \caption{Static filter $f$=1, are three jobs are filtered.}\label{fig:af2-4}
\end{subfigure}
\caption{Themis Example B (Table~\ref{tab:example_filter_2}). Comparing adaptive filter with static filter.  In each round, the jobs filtered or selected for allocation are shaded. Nonshaded jobs in each round are work-conserving jobs that receive left-over GPUs that are not allocated to the filtered jobs (see leftover allocation in Themis\cite{themis20}). Cluster setting: 4 GPUs. Jobs: A, B, and C are three DNN training jobs with one iteration. Serial iteration times for A, B, and C are 12, 8 and 4, respectively. The number of requested GPUs per iteration for A, B, and C is 3, 2, and 4, respectively. As assumed in Themis \cite{themis20}, we adopt a linear slowdown per iteration when the number of allocated GPUs is less than requested.}\label{fig:adaptive_vs_static_filter_2}
\end{figure*}

==> apdx_simulation_fidelity.tex <==
\section{Simulation Fidelity}\label{apdx:fidelity}
\input{tab-policy-sim-fidelity}
Overall, the results on physical cluster are in agreement with results in simulation. In Table~\ref{tab:fidelity2}, we report the simulation fidelity of the 32-GPU cluster experiments by presenting the (relative) differences in end-to-end objectives between physical runs and simulations. Similar to Pollux~\cite{qiao2020pollux}, we also simulate the overhead of checkpoint-restarts and inject a 20-second delay for jobs that are re-scheduled across rounds. The differences between physical and simulation across policies and metrics have an average of 4.5\% and a maximum of 9.9\%, which are on par with the fidelity reported in Gavel \cite{gavel20}. 

==> apdx_welfare_example.tex <==
\section{Examples - Social Welfare Over Time and Efficiency-Fairness Trade-off}\label{apdx:MNSW-example}

Maximized social welfare (over time) balances efficiency and fairness. The intuition behind is explained with examples as below. 

(1) \textit{Fairness - Starvation Free.} Within each shot of scheduling, maximized Nash social welfare minimizes the possibility that a job gets starved. If a job has zero or very low progress percentage (i.e., zero or low job utility), the log utility for the job approaches negative infinite, and the integrated social welfare at cluster level will not reach its maximum. 

(2) \textit{Fairness - Compensation of Unfairness in the Past - The Power of Diminishing Returns.} The social welfare function rejects the phenomenon "the richer get richer and the poorer get poorer". It rebalances jobs' progress using diminishing return of log function. That is, allocating the same amount of resource to a job with higher progress percentage increases utility less than allocating that to another job with lower progress percentage.

\textit{\textbf{Example A. - A case for significant unfairness - Stopping enriching the rich and compensating the poor.} Before a shot of scheduling, suppose that a ``rich'' Job A gets 80\% percentage of epoch progresses already and another ``poor'' Job B gets only 20\%. Suppose the planning window is of 5 rounds and each of the jobs makes a 1\% epoch progress per round. Due to resource limits, only a single job can be scheduled per round. For example, if the schedules run Job B for 4 rounds with a 4\% epoch progress increase, then Job A will receive only one round for a 1\% epoch progress. The resulting social welfare for different schedules is listed in Table~\ref{example:sw1}. The result show that, for this case, social welfare is maximized when scheduling Job B for all of the 5 rounds to compensate for this lagged progress compared with A.} 


\begin{table}[htbp!]
\begin{tabularx}{\columnwidth}{c c X X X X X}
    \hline
    \makecell[c]{(Job A, Job B)\\ Schedule}& \makecell[l]{(5, 0)} & \makecell[l]{(4, 1)}& \makecell[l]{(3, 2)}& \makecell[l]{(2, 3)}& \makecell[l]{(1, 4)} & \makecell[l]{(0, 5)}\\[-5pt]
    \hline
    \makecell[l]{Social Welfare}& \makecell[l]{-1.34} & \makecell[l]{-1.02}& \makecell[l]{-0.82}& \makecell[l]{-0.69}& \makecell[l]{-0.62} & \makecell[l]{-0.58}\\[-10pt]
    \hline
\end{tabularx}
\caption{\label{example:sw1} Example - Social Welfare. The first line indicates the allocation of rounds (5 in total) for Job A (left) and B (right). The second line shows the resulting social welfare.}
\end{table}

\begin{table}[htbp!]
\begin{tabularx}{\linewidth}{c c X X X X X}
    \hline
    \makecell[c]{(Job A, Job B)\\ Schedule}& \makecell[l]{(5, 0)} & \makecell[l]{(4, 1)}& \makecell[l]{(3, 2)}& \makecell[l]{(2, 3)}& \makecell[l]{(1, 4)} & \makecell[l]{(0, 5)}\\[-5pt]
    \hline
    \makecell[l]{Social Welfare}& \makecell[l]{-1.61} & \makecell[l]{-1.31}& \makecell[l]{-1.14}& \makecell[l]{-1.05}& \makecell[l]{-1.02} & \makecell[l]{-1.05}\\[-10pt]
    \hline
\end{tabularx}
\caption{\label{example:sw2} Example - Social Welfare. The first line indicates the allocation of rounds (5 in total) for Job A (left) and Job B (right). The second line shows the resulting social welfare.}
\end{table}

(3) \textit{Balancing Efficiency and Fairness.} The social welfare function does not simply compensate for unfairness in past scheduling rounds; it tries to maximize the cluster-wide efficiency given a moderate degree of unfairness. See the example below. 

\textit{\textbf{Example B - A case for efficiency and fairness balance - Enriching all.} Before a shot of scheduling, suppose a ``middle-class'' Job A get 50\% percentage of epoch progresses already and another ``poor'' Job B gets only 20\%. Suppose that the planning window is of 5 rounds and each of the jobs makes a 1\% epoch progress per round. Due to resource limits, only a single job can be scheduled per round. The resulting social welfare for different schedules is listed in Table~\ref{example:sw2}. The result show that, for this case, social welfare is maximized when scheduling Job B for 4 out of the 5 rounds, and schedule job A for 1 round. Maximized social welfare tries to improved the progress of all jobs at the cluster level when unfairness in the past is to a moderate degree.} 



==> discussion.tex <==
\color{blue}
\section{Discussion.}

\textbf{Why not apply reinforcement learning for proactive scheduling?} Economic theory offers provable guarantees of efficiency and fairness, while reinforcement learning \cite{mao_rl_sigcomm19} typically does not. Nevertheless, \project also applies ML (Bayesian) models to forecast batch size changes. Incorporating different learners into \project, as well its comparison against RL, is important future work.

\textbf{Why not apply hyperparmaeter tuning to tune the fairness knob $f$ in Themis and AlloX?} Hyperparameter tuning is typically performed using multi-arm bandit methods; to apply them, many scheduler instances, each with a different filter $f$, need to be spawned to collect trial-and-error data. This will require orders of magnitude more system resources. \project avoids expensive filter tuning and optimizes elastic resource allocation over time.

\textbf{Practicability of \project.} \project commits a lot of efforts in translating economic theories to practical systems. First, it is computationally intractable to optimize Nash social welfare for (infinitely) long future. At a practical level, \project efficiently optimizes social welfare for a finite future, and construct estimators for long-term fairness and efficiency to in substitution of long-term welfare. Second,\project’s equilibrium solution is relaxed to a simple linear integer program, which can be efficiently solved using existing solvers (e.g., Gurobi). Our evaluation also shows \project has low overhead and scales to large clusters. Second, \project’s dynamic adaptation model draws on domain and expert knowledge, and has a simple analytical form that can be re-estimated in real time to capture system dynamics. Third, \project's prediction errors in dynamic adaption are relatively low (\ref{fig:dirichlet}). The errors cause only a small fraction of jobs to break fairness, and the worst-case unfairness is not significantly affected.

\color{black}



==> eval_hparam_sensitivity.tex <==
\subsection{Hyperparameter Effect}\label{subsec:hparam}
\shivaram{we can move this to appendix}
\project has two hyperparameters, the length of the planning window, i.e., $w$, and the regularizer $\lambda$ that controls the strength of the efficiency heuristic. A larger $w$ renders more future exploration and farsighted scheduling but suffers from an inaccurate prediction of the long future. A larger $\lambda$ advocates \project to opportunistically prioritize long jobs that dominate makespan. 
\begin{figure}[htbp!]
  \includegraphics[width=0.9\linewidth]{figures/hparam.png}
  \caption{Hyperparameter Effect Analysis. Default $w$= 1Hr and default $\lambda$=5e-1 ($\lambda_0$).} \label{fig:hparam}
\end{figure}
First, we tune $w$ from 10 minutes to 2 hours to study the effect of future exploration.  Figure~\ref{fig:hparam} shows that a medium window length of one-hour yields best makespan and fairness, while a short window of 10 minutes and a large window of 2 hours are worse. Medium window length trades-off the benefits of future exploration and the risks in inaccurate future prediction. 

Second, we tune $\lambda$ in log-space over four orders of magnitude, while fixing the window length as one hour, \project exhibits similar makespan and fairness when tuning $\lambda$ around the default value, i.e., between $\frac{\lambda_0}{4}$ and $32\lambda_0$. But a very small $\lambda$ ($<\frac{\lambda_0}{16}$) prolongs makespan and a very large $\lambda$ ($>32\lambda_0$) degrades fairness. We recommend setting $w$=1 Hr and $\lambda=\lambda_0$, which is repeatedly used in our experiments.

==> tab-policy-sim-fidelity.tex <==

\begin{table*}[htbp!]
\begin{center}
\begin{tabular}{ |c|c|c|c| } 
 \hline
 Policy\textbackslash Metric & Makespan (\% diff) & Avg JCT (\% diff) & Unfair fraction (abs. diff) \\ 
 \hline 
 Shockwave & 7.97 & 5.69 & 8.0 \\ 
 \hline
 OSSP & 1.23 & 1.95 & 2.0 \\ 
 \hline
 Themis & 0.02 & 0.82 & 2.0 \\ 
 \hline
 Gavel & 4.69 & 9.2 & 7.0 \\ 
 \hline
 AlloX & 6 & 8.02 & 0.01 \\ 
 \hline
 MST & 9.92 & 2.02 & 4.0 \\ 
 \hline
 Average & 4.97 & 4.62 & 3.83 \\ 
 \hline 
\end{tabular}
\caption{\label{tab:fidelity2}Per-policy simulation fidelity of running 120-job traces in a 32-GPU shared cluster. For makespan (s) and average JCT (s), we report the relative difference, and for unfair fraction (\%), we report the absolute difference.}
\end{center}
\end{table*}

